NeRF-US: Removing Ultrasound Imaging Artifacts from Neural Radiance Fields in the Wild

Current methods for performing 3D reconstruction and novel view synthesis (NVS) in ultrasound imaging data often face severe artifacts when training NeRF-based approaches. The artifacts produced by current approaches differ from NeRF floaters in general scenes because of the unique nature of ultrasound capture. Furthermore, existing models fail to produce reasonable 3D reconstructions when ultrasound data is captured or obtained casually in uncontrolled environments, which is common in clinical settings. Consequently, existing reconstruction and NVS methods struggle to handle ultrasound motion, fail to capture intricate details, and cannot model transparent and reflective surfaces. In this work, we introduced NeRF-US, which incorporates 3D-geometry guidance for border probability and scattering density into NeRF training, while also utilizing ultrasound-specific rendering over traditional volume rendering. These 3D priors are learned through a diffusion model. Through experiments conducted on our new "Ultrasound in the Wild" dataset, we observed accurate, clinically plausible, artifact-free reconstructions.

==> preamble.tex <==
\RequirePackage{graphicx}
\usepackage{layouts}
 % The following packages will be automatically loaded:
 % amsmath, amssymb, natbib, graphicx, url, algorithm2e
 \usepackage{booktabs}
 %\usepackage{rotating}% for sideways figures and tables
\usepackage{longtable}% for long tables
 % The booktabs package is used by this sample document
 % (it provides \toprule, \midrule and \bottomrule).
 % 
 % book quality tables

 % The siunitx package is used by this sample document
 % to align numbers in a column by their decimal point.
 % Remove the next line if you don't require it.
\makeatletter
\def\set@curr@file#1{\def\@curr@file{#1}} %temp workaround for 2019 latex release
\makeatother
\usepackage[load-configurations=version-1]{siunitx} % newer version
\usepackage{xspace}
\usepackage{lipsum}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{bbding}
\usepackage{floatrow}
\ifdefined\layout
    \usepackage{layouts}
\fi
\usepackage[most]{tcolorbox}
\usepackage{cleveref}
\usepackage{overpic}
% \usepackage[nobottomtitles]{titlesec}
\usepackage{cancel}
\usepackage{currfile}
\usepackage{diagbox}
\usepackage{algpseudocode}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage[nice]{nicefrac}
\usepackage{algpseudocode}

 % The following command is just for this sample document:
\newcommand{\cs}[1]{\texttt{\char`\\#1}}
\newcommand{\acronym}{NeRF-US}
\newcommand{\acronymtitle}{NeRF-US}
\newcommand{\website}{rishitdagli.com/nerf-us/}
\newcommand*\us{\vcenter{\hbox{\includegraphics[height=\baselineskip]{figures/emoji.png}}}}

 % Define an unnumbered theorem just for this sample document:
\theorembodyfont{\upshape}
\theoremheaderfont{\scshape}
\theorempostheader{:}
\theoremsep{\newline}
\newtheorem*{note}{Note}

\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow
\definecolor{vlet}{rgb}{0.95, 0.6, 0.95}

\def\arxiv{}
% \def\submission{}
% \def\cameraready{}

% \def\layout{}

\ifdefined\submission
    \jmlrvolume{[VOLUME \# TBD]}
    \jmlryear{2024}
    \jmlrworkshop{Machine Learning for Healthcare}
\fi
\ifdefined\arxiv
    \jmlrvolume{}
    \jmlryear{2024}
    \jmlrworkshop{}
\fi
\ifdefined\cameraready
    \jmlrvolume{252}
    \jmlryear{2024}
    \jmlrworkshop{}
\fi
\newif\ifarxivorcameraready
\ifdefined\arxiv
  \arxivorcamerareadytrue
\fi
\ifdefined\cameraready
  \arxivorcamerareadytrue
\fi

\title[\acronym]{\acronymtitle $\us$\ : Removing Ultrasound Imaging Artifacts \\from Neural Radiance Fields in the Wild}

\ifdefined\submission
    \author{\Name{Anonymous Author(s)}\\
           % \Email{name@email.edu}\\ 
           \addr Under Review
    % \\\\\Name{\href{https://\website}{\url{\website}}}
    }
\fi
\ifarxivorcameraready
    \author{\Name{Rishit Dagli} $^{1,2}$ \Email{rishit@cs.toronto.edu}\\
    \Name{Atsuhiro Hibi} $^{2,3,4}$ \Email{atsuhiro.hibi@mail.utoronto.ca}\\
    \Name{Rahul G. Krishnan} $^{1,5}$ \Email{rahulgk@cs.toronto.edu}\\
    \Name{Pascal N. Tyrrell} $^{2,4,6}$ \Email{pascal.tyrrell@utoronto.ca}
    \AND
    \addr Departments of~$^1$ \addr Computer Science;
    $^2$ \addr Medical Imaging, University of Toronto, Canada\\
    $^3$ \addr Division of Neurosurgery, St Michael's Hospital, Unity Health Toronto, Canada\\
    $^4$ \addr Institute of Medical Science; Departments of~$^5$ \addr Laboratory Medicine and Pathobiology; $^6$ \addr Statistical Sciences, University of Toronto, Canada\\
    \\\\
    \Name{\href{https://\website}{\url{\website}}}
    }
\fi
